Multimodal Optimization with k-Cluster Big Bang-Big Crunch Algorithm and Postprocessing Methods for Identification and Quantification of Optima

Multimodal optimization is often encountered in engineering problems, especially when different and alternative solutions are sought. Evolutionary algorithms can efficiently tackle multimodal optimization thanks to their features such as the concept of population, exploration/exploitation, and being suitable for parallel computation. This paper investigates whether a less-known optimizer, the Big Bang-Big Crunch (BBBC) algorithm, is suitable for multimodal optimization. We extended BBBC and propose k-BBBC, a clustering-based multi-modal optimizer. Additionally, we introduce two post-processing methods to (i) identify the local optima in a set of retrieved solutions (i.e., a population), and (ii) quantify the number of correctly retrieved optima against the expected ones (i.e., success rate). Our results show that k-BBBC performs well even with problems having a large number of optima (tested on $379$ optima) and high dimensionality (tested on $32$ decision variables), but it becomes computationally too expensive for problems with many local optima (i.e., in the CEC'2013 benchmark set). Compared to other multimodal optimization methods, it outperforms them in terms of accuracy (in both search and objective space) and success rate (number of correctly retrieved optima) when tested on basic multimodal functions, especially when elitism is applied; however, it requires knowing the number of optima of a problem, which makes its performance decrease when tested on niching competition test CEC'2013. Lastly, we validated our proposed post-processing methods by comparing their success rate to the actual one: results suggest that these methods can be used to evaluate the performance of a multimodal optimization algorithm by correctly identifying optima and providing an indication of success -- without the need to know where the optima are located in the search space.

==> tableFunctions.tex <==
% Table with the functions -- Part 1
\begin{table*}[]
\centering
\caption{Benchmark Problems (1/3)}
\label{tab:bench_functions}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cccccccc|}
\hline
\textbf{Function} & \textbf{Type} & \textbf{Bounds} & \makecell{\textbf{Dimensions}\\$(d)$} & \makecell{\textbf{Optima}\\$(m)$} & \makecell{\textbf{Clusters}\\($k$)} & \makecell{\textbf{Population Size}\\($n$)} & \textbf{Graph} \\ \hline

\begin{tabular}{l}
\makecell{Rollercoaster \\ $f_1(\textbf{x}) = 2^{-2(\frac{x-0.1}{0.8})^2}\cdot \sin{5 \pi x}^6$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{max} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[0,1\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$1$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$5$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$10$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$200$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_rollercoaster.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Key4 \\ $f_2(\textbf{x}) = {10 (1+\cos{(2 \pi 4 x)}) + 8 x^2}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[0,1\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$1$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$4$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$8$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$160$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_key4.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Key8 \\ $f_3(\textbf{x}) = {10 (1+\cos{(2 \pi 8 x)}) + 16 x^2}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[0,1\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$1$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$8$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$16$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$320$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_key8.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Key16 \\ $f_4(\textbf{x}) = {10 (1+\cos{(2 \pi 16 x)}) + 32 x^2}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[0,1\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$1$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$16$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$32$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$640$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_key16.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Key24 \\ $f_5(\textbf{x}) = {10 (1+\cos{(2 \pi 24 x)}) + 48 x^2}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[0,1\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$1$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$24$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$48$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$960$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_key24.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Key48 \\ $f_6(\textbf{x}) = {10 (1+\cos{(2 \pi 48 x)}) + 96 x^2}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[0,1\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$1$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$48$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$96$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$1920$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_key48.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Key96 \\ $f_7(\textbf{x}) = {10 (1+\cos{(2 \pi 96 x)}) + 192 x^2}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[0,1\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$1$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$96$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$192$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$3840$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_key96.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Schwefel \\ $f_8(\textbf{x}) = 418.9829 - x \sin{(\sqrt{|x|})}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-500,500\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$1$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$8$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$16$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$320$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_schwefel1d.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Schwefel \\ $f_9(\textbf{x}) = 2 \cdot 418.9829 - \sum_{i=1}^{2}{x_i\sin{(\sqrt{|x_i|})}}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-500,500\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$64$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$256$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$5120$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_schwefel.pdf}}
\end{tabular}
\\ \hline

\end{tabular}%
}
\end{table*}

% Table with the functions -- Part 2 ------------------------------------------------------------------------------------
\begin{table*}[]
\centering
\captionsetup{labelformat=empty}
\caption{Benchmark Problems (2/3)}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cccccccc|}
\hline
\textbf{Function} & \textbf{Type} & \textbf{Bounds} & \makecell{\textbf{Dimensions}\\$(d)$} & \makecell{\textbf{Optima}\\$(m)$} & \makecell{\textbf{Clusters}\\($k$)} & \makecell{\textbf{Population Size}\\($n$)} & \textbf{Graph} \\ \hline

\begin{tabular}{l}
\makecell{Himmelblau \\ $f_{10}(\textbf{x}) = {({x_1}^2 + x_2 - 11)^2 +(x_1 + {x_2}^2 - 7)^2}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-6,6\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$4$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$16$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$320$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_himmelblau.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Bird \\ $f_{11}(\textbf{x}) = {\sin(x_1)\exp(1 - \cos{x_2})^2 +}  $ \\ ${+\cos{x_2}\exp(1 - \sin{x_1})^2 + (x_1 - x_2)^2}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-2\pi,2\pi\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$4$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$16$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$320$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_bird.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Rastrigin \\ $f_{12}(\textbf{x}) = {20 + {x_1}^2 + {x_2}^2 } - $ \\${- 10(\cos{(2\pi x_1)} + \cos{(2\pi x_2)})}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-5.12,5.12\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$121$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$484$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$9680$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_rastrigin.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Cosine Mixture \quad $f_{13}(\textbf{x}) = $ \\ $ {-(0.2 + {x_1}^2 + {x_2}^2 - 0.1\cos{(6\pi x_1)} - 0.1. \cos{(6 \pi x_2)})}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-1,1\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$25$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$100$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$2000$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_cosineMixture.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Cross-in-Tray \quad $f_{14}(\textbf{x}) =$ \\ $ {-(10^{-4}\abs{\sin{x_1}\sin{x_2}\exp(\abs{100 - \frac{\sqrt{{x_1}^2 + {x_2}^2}}{\pi}})} + 1)^{0.1}}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-9.5,9.5\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$36$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$144$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$2880$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_crossintray.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Vincent \\ $f_{15}(\textbf{x}) = {-(\sin{(10\log{x_1})} + \sin{(10\log{x_2})})}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[0.25,10\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$36$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$144$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$2880$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_vincent.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Holder Table \\ $f_{16}(\textbf{x}) = {-\abs{\sin{x_1}\cos{x_2}\exp(\abs{1 - \frac{\sqrt{{x_1}^2 + {x_2}^2}}{\pi}})}}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-10,10\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$56$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$224$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$4480$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_holdertable.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Pen Holder \quad $f_{17}(\textbf{x}) =$ \\ $ {-\exp(-|\cos{x_1}\cos{x_2}\cdot \exp(\abs{1 - \frac{\sqrt{{x_1}^2 + {x_2}^2}}{\pi}})|^{-1})}$}
%${\cdot \exp(\abs{1 - \frac{\sqrt{{x_1}^2 + {x_2}^2}}{\pi}})|^{-1})}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{max} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[0,1\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$49$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$196$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$3920$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_penholder.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Egg Crate \\ $f_{18}(\textbf{x}) = {{x_1}^2 + {x_2}^2 + 25(\sin{x_1}^2 + \sin{x_2}^2)}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-5,5\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$9$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$36$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$720$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_eggcrate.pdf}}
\end{tabular}
\\ \hline

\end{tabular}%
}
\end{table*}

% Table with the functions -- Part 3 ------------------------------------------------------------------------------------
\begin{table*}[]
\centering
\captionsetup{labelformat=empty}
\caption{Benchmark Problems (3/3)}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cccccccc|}
\hline
\textbf{Function} & \textbf{Type} & \textbf{Bounds} & \makecell{\textbf{Dimensions}\\$(d)$} & \makecell{\textbf{Optima}\\$(m)$} & \makecell{\textbf{Clusters}\\($k$)} & \makecell{\textbf{Population Size}\\($n$)} & \textbf{Graph} \\ \hline

\begin{tabular}{l}
\makecell{Griewank \\ $f_{20}(\textbf{x}) = {\frac{{x_1}^2 + {x_2}^2}{4000} - \cos{x}\cos{(\frac{x_2}{\sqrt{2}})} + 1}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{min} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-50,50\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$379$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$1516$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$30320$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_griewank.pdf}}
\end{tabular}
\\ \hline

\begin{tabular}{l}
\makecell{Griewank \\ $f_{20}(\textbf{x}) = {-\frac{{x_1}^2 + {x_2}^2}{4000} + \cos{x}\cos{(\frac{x_2}{\sqrt{2}})} - 1}$}
\end{tabular}
& 
\begin{tabular}{l}
\texttt{max} % type
\end{tabular}
& 
\begin{tabular}{l}
$\left[-50,50\right]$ % bounds
\end{tabular}
& 
\begin{tabular}{l}
$2$ % dimensions
\end{tabular}
&
\begin{tabular}{l}
$379$ % num of optima
\end{tabular}
&
\begin{tabular}{l}
$1516$ % num of clusters
\end{tabular}
&
\begin{tabular}{l}
$30320$ % pop size
\end{tabular}
&
\begin{tabular}{l}
\raisebox{-\totalheight}{\includegraphics[height=2.5cm]{figures/fun_griewankmax.pdf}}
\end{tabular}
\\ \hline

\end{tabular}%
}
\end{table*}
